DeepProbe: Information Directed Sequence Understanding and Chatbot Design via Recurrent Neural Networks

Information extraction and user intention identification are central topics in modern query understanding and recommendation systems. In this paper, we propose DeepProbe, a generic information-directed interaction framework which is built around an attention-based sequence to sequence (seq2seq) recurrent neural network. DeepProbe can rephrase, evaluate, and even actively ask questions, leveraging the generative ability and likelihood estimation made possible by seq2seq models. DeepProbe makes decisions based on a derived uncertainty (entropy) measure conditioned on user inputs, possibly with multiple rounds of interactions. Three applications, namely a rewritter, a relevance scorer and a chatbot for ad recommendation, were built around DeepProbe, with the first two serving as precursory building blocks for the third. We first use the seq2seq model in DeepProbe to rewrite a user query into one of standard query form, which is submitted to an ordinary recommendation system. Secondly, we evaluate DeepProbe's seq2seq model-based relevance scoring. Finally, we build a chatbot prototype capable of making active user interactions, which can ask questions that maximize information gain, allowing for a more efficient user intention idenfication process. We evaluate first two applications by 1) comparing with baselines by BLEU and AUC, and 2) human judge evaluation. Both demonstrate significant improvements compared with current state-of-the-art systems, proving their values as useful tools on their own, and at the same time laying a good foundation for the ongoing chatbot application.

==> implementation.tex <==
\section{Implementation and Experiments}\label{implementation}

In this chapter, we describe our implementation of the ad recommendation chatbot, and discuss some of the key hacks about the main framework to make it compatible with the current system.\\
As discussed in chapters \ref{Bayesian}, in order to calculate the conditional distribution of ads given a query $Q$, it is required that the likelihood $P(Q|Ad)$ be computed for every $Ad\in\mathcal A$. This issue was present in all other proposed information retrieval systems based on statistical language models, demanding a $O(|\mathcal A|)$ complexity. When $|\mathcal A|$ is large, This poses challenges on both the system side, considering the number of queries, and quality of service, as the chatbot is expected to be responsive and should not wait too long before return the next action.

==> training.tex <==
\section{Training}\label{training}

We present some training detail of the seq2seq likelihood estimator. In addition to likelihood estimation, this same model has the ability to perform query rewriting task, which will be discussed in section \ref{application}.

\subsection{Data Description}
The seq2seq model was trained on our internal dataset, which consists of clicked (offer, query) pairs. The offers come from a product ad database, each is a sequence of words describing the corresponding product. The queries are user inputs in our search engine, and if the user clicked on an offer when searching with a query, we regard it as a valid (offer, query) pair. A total of 100 million such training pairs were collected.

\subsection{Details of Model}
We used the model introduced in section \ref{seq2seq}, with vocabulary size $|\mathcal V|=30k$. Any word that is not part of $\mathcal V$ is assigned with symbol $\langle$UNK$\rangle$. We chose the embedding dimension $d=300$. On the encoder side, we used bi-directional LSTM network with a total of 4 vertically stacked layers. At the decoder side, 4-layer LSTM network was used, and we implemented 4 different attention scenarios: no attention, cosine similarity weighted average as in \cite{luong-pham-manning:2015:EMNLP}, general matrix similarity weighted average as in \cite{luong-pham-manning:2015:EMNLP}, and our dynamic tensor attention network. The results for the four different attention mechanisms are compared. 

We used Theano \cite{2016arXiv160502688short} for model training on a Tesla K20 GPU. We used cross entropy as the loss function, and Adadelta \cite{zeiler2012adadelta} for gradient descent, which is a variant of Adagrad \cite{duchi2011adaptive}. We trained the model for 5? epochs, each epoch takes 3? days. 


